Bridging Both Worlds in Semantics and Time: Domain Knowledge Based Analysis and Correlation of Industrial Process Attacks

Modern industrial control systems (ICS) attacks infect supervisory control and data acquisition (SCADA) hosts to stealthily alter industrial processes, causing damage. To detect attacks with low false alarms, recent work detects attacks in both SCADA and process data. Unfortunately, this led to the same problem - disjointed (false) alerts, due to the semantic and time gap in SCADA and process behavior, i.e., SCADA execution does not map to process dynamics nor evolve at similar time scales. We propose BRIDGE to analyze and correlate SCADA and industrial process attacks using domain knowledge to bridge their unique semantic and time evolution. This enables operators to tie malicious SCADA operations to their adverse process effects, which reduces false alarms and improves attack understanding. BRIDGE (i) identifies process constraints violations in SCADA by measuring actuation dependencies in SCADA process-control, and (ii) detects malicious SCADA effects in processes via a physics-informed neural network that embeds generic knowledge of inertial process dynamics. BRIDGE then dynamically aligns both analysis (i and ii) in a time-window that adjusts their time evolution based on process inertial delays. We applied BRIDGE to 11 diverse real-world industrial processes, and adaptive attacks inspired by past events. BRIDGE correlated 98.3% of attacks with 0.8% false positives (FP), compared to 78.3% detection accuracy and 13.7% FP of recent work.

==> tables/scenarios-changed.tex <==
\begin{table*}[t]
    \centering
    \footnotesize
    \resizebox{0.95\textwidth}{!}{
        \begin{tabular}{@{}|l|c|ccc|>{\columncolor[gray]{0.9}}c>{\columncolor[gray]{0.9}}l|>{\columncolor[gray]{0.9}}c|>{\columncolor[gray]{0.9}}c>{\columncolor[gray]{0.9}}c>{\columncolor[gray]{0.9}}c|ccc|c|cccc|@{}}
            \toprule
            %\cline{1-20}
            Industrial&Diverse& \multicolumn{3}{c|}{OPC Events}& \multicolumn{6}{c}{\scada Process-Control Dependency Analysis} & \multicolumn{3}{|c|}{Process Constraints} &&\multicolumn{4}{c|}{Process Behavior}\\
             \cline{6-11} 
               Processes&Domains&\multicolumn{3}{c|}{(Per Process)}&\multicolumn{3}{|c|}{Process Function and Relevant Actuators}&\multicolumn{3}{c}{Proc Graph} & \multicolumn{3}{|c|}{(Statistical Averages)}& & \multicolumn{4}{c|}{(PINN/PDE Training)} \\  
            \cline{3-14}
            \cline{16-19}
            && \rotatebox{90}{Scenario} \rotatebox{90}{FileSize} &\rotatebox{90}{States} & \rotatebox{90}{Verify} &Description &\rotatebox{90}{Task ID}& Key Actuator  &\rotatebox{90}{CMDs} &\rotatebox{90}{Nodes} &\rotatebox{90}{Edges}  &$R_{D\Delta}$ & $R_{D\mu}$ & $R_{D\digamma}$& \rotatebox{90}{Analysis} \rotatebox{90}{Time (m)} &\rotatebox{90}{Inertia/}\rotatebox{90}{Seq Size} &\rotatebox{90}{Precision} &\rotatebox{90}{Recall} &\rotatebox{90}{F1} \\
            \cline{1-19} 
            \rowcolor{Gray}
            &&11.5K &10 &0&level control&2.1 &holding tank &24 &4 &6 &0.47 &0.125 &0.105 &7.6  &4.5/5&85&70&77\\
            \rowcolor{Gray}
           \multirow{-2}{*}{Chemical Dosing}&\multirow{-2}{*}{Water Treatm} &11.5K &14 &2& dosing&2.2 &dose valve &22 &5 &9 &0.419 &0.111 &0.344 &7.5   &4.5/5&94&87&90\\
            
            &&29K &20 &0&pallet alignment&3.2 &Axes X,Z &26 &6  &4 &0.41 &0.133 &0.088 &12.4  &5.1/5&95&93&94\\
           \multirow{-2}{*}{Auto warehouse}&\multirow{-2}{*}{Manufacture} &29K &36 &1& throughput&3.2 &entry conveyor &32 &7 &5 &0.42 &0.167 &0.034 &12.9   &5.1/6&77&83&80\\
           
           \rowcolor{Gray}
           &&9.5K &28 &0&product haul&4.1 &clamp lid/base &22 &5 &9 &0.24 &0.71 &0.048 &7.7   &5.7/6&71&73&72\\
            \rowcolor{Gray}
           \multirow{-2}{*}{Assembler}&\multirow{-2}{*}{Manufacture} &9.5K &11 &1& load balancing&4.2 &conveyor2 &17 &4  &3 &0.686 &0.14 &0.05 &9.3   &5.1/6&88&93&90\\
                        
            &&11K &13 &0 &prod safety&11.1 &conveyor1-3 &25 &6 &6 &0.198 &0.195 &0.51 &12.0 &7.4/7&92&85&88\\
           \multirow{-2}{*}{Elevator}&\multirow{-2}{*}{Manufacture}&11K &12 &0 & throughput&11.2  &entry conveyor &14 &8 &5  &0.318 &0.119 &0.691 &6.1   &7.4/7&89&77&83\\

           
           
           \rowcolor{Gray}
           &&9K &12 &0 &spacing &7.1&buffer conveyor &17 &4 &5 &0.091 &0.089 &0.441 &4.7  &6.4/6&82&90&86\\
            \rowcolor{Gray}
           \multirow{-2}{*}{Queue processor}&\multirow{-2}{*}{Manufacture} &9K &29 &0& throughput &7.2 &entry conveyor &32 &8 &4 &0.358 &0.678 &0.224 &12.1   &6.4/6&88&95&91\\

            &&6K &18 &0 &heat setpoint &6.1&room temp &9 &4 &5 &0.219 &0.053 &0.09 &11.6  &11.8/13&79&92&85\\
           \multirow{-2}{*}{HVAC}&\multirow{-2}{*}{A/C} &6K &17 &1& heat flow&6.2 &vent &23 &5 &5 &0.178 &0.410 &0.065 &10.2   &11.8/13&88&83&85\\
            \rowcolor{Gray}
           
            &&7.8K &21 &1&load alignment&5.1 &push clamp &33 &9  &4 &0.289 &0.845 &0.717 &14.6  &4.1/4&80&88&84\\
            \rowcolor{Gray}
           \multirow{-2}{*}{Palletizer}&\multirow{-2}{*}{Shipping} &7.8K &29 &0 & prod protection&5.2 &entry conveyor &36 &6 &7 &0.091 &0.459 &0.455 &5.8  &4.1/8&71&79&75\\
            %&  &19K &19 &0&load balancing&1.1 &c-breaker &13 &7 &6 &0.265 &0.341 &0.52 &6.7  \\
            
            %\multirow{-2}{*}{Power} &\multirow{-2}{*}{Power} &11K &21 &0&line distribution&1.2 &load lines &11 &7  &5 &0.651 &0.195 &0.134&16.0   \\
            &&6.2K &11 &1&path throughput&7.1 &load/unload &32 &7 &5  &0.421 &0.616 &0.321 &9.5   &5.1/6&86&93&89\\
           \multirow{-2}{*}{Converge station} &\multirow{-2}{*}{Shipping} &6.2K &19 &0& alt throughput&7.2 &transfer &23 &9  &8  &0.51 &0.18 &0.085 &11.4  &5.1/6&88&93&90\\
           \rowcolor{Gray}
           &&8.5K &21 &1&alignment&4.1 &control arm &22 &8 &6 &0.267 &0.371 &0.571 &11.3   &12.1/12&84&99&91\\
            \rowcolor{Gray}
           \multirow{-2}{*}{Production line}&\multirow{-2}{*}{Manufacture}&8.5K &11 &0 & throughput&8.2 &conveyors &25 &5 &5 &0.211  &0.098 &0.0510 &9.9   &12.1/12&66&94&78\\
            
            &&9K &16 &0&sort accuracy&9.1 &unloader &22 &8 &7 &0.4 &0.335 &0.118 &15.1  &5.5/6&92&93&92\\
           \multirow{-2}{*}{Sort station}&\multirow{-2}{*}{Shipping} &9K &16 &0& throughput&9.2 &conveyor &17 &9 &5 &0.107 &0.291 &0.0821 &10.6  &5.5/6&97&70&89\\
           
           \rowcolor{Gray}
           &&4.9K &18 &0&accuracy &10.1 &pusher1-2 &26 &11 &8 &0.132 &0.439 &0.264 &12.0   &7.6/8&89&73&81\\
            \rowcolor{Gray}
           \multirow{-2}{*}{Separator}&\multirow{-2}{*}{Shipping} &4.9K &15 &0& throughput&10.2 &conveyors &27 &8  &7 &0.414 &0.193 &0.072 &9.6  &7.6/8&86&86&80\\
           \bottomrule
        \end{tabular}
    }
    \caption{Showing \sys's analysis results per process based on public dataset of diverse real-world industrial processes.}
    \label{tbl:scenarios}
\end{table*}
